Dramatic pressure-induced slowdown and the soft glassy rheology of water at 2D material interface

The flow of molecularly confined water has attracted considerable interest in recent years. Yet despite their exquisite character, current nanofluidic devices cannot probe molecular water flow beyond the linear-response regime, while nanomechanical force- based approaches have produced markedly inconsistent results. Here, using tuning- fork-based atomic force microscopy, we tackle these limitations by measuring the full linear-to-nonlinear, shear-dependent viscoelastic rheology of molecularly confined water at various two-dimensional material interfaces -- demonstrating pronounced rate effects in water flow response. The observed rheological behaviors are remarkably analogous to that of macroscopic soft glassy yielding materials and fully captured by a non-linear model accounting for the shear-induced acceleration of the dynamics -- a hallmark of disordered supercooled and metastable systems. We further unveil a pronounced pressure-induced slowdown in nanoconfined water dynamics, with relaxation times extending into the microsecond range and marked material dependence. These results reveal non-linear, glassy rheology as a general feature of interfacial water and offer a route to tunable, non-linear nanofluidic elements.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
